A Novel Evaluation Perspective on GNNs-based Recommender Systems through the Topology of the User-Item Graph

Recently, graph neural networks (GNNs)-based recommender systems have encountered great success in recommendation. As the number of GNNs approaches rises, some works have started questioning the theoretical and empirical reasons behind their superior performance. Nevertheless, this investigation still disregards that GNNs treat the recommendation data as a topological graph structure. Building on this assumption, in this work, we provide a novel evaluation perspective on GNNs-based recommendation, which investigates the impact of the graph topology on the recommendation performance. To this end, we select some (topological) properties of the recommendation data and three GNNs-based recommender systems (i.e., LightGCN, DGCF, and SVD-GCN). Then, starting from three popular recommendation datasets (i.e., Yelp2018, Gowalla, and Amazon-Book) we sample them to obtain 1,800 size-reduced datasets that still resemble the original ones but can encompass a wider range of topological structures. We use this procedure to build a large pool of samples for which data characteristics and recommendation performance of the selected GNNs models are measured. Through an explanatory framework, we find strong correspondences between graph topology and GNNs performance, offering a novel evaluation perspective on these models.

==> figures/lgcn_gowalla.tex <==
\begin{tikzpicture}
  \begin{axis}[,
    xbar,
    y axis line style = { opacity = 0 },
    axis x line       = none,
    tickwidth         = 0pt,
    ytick             = data,
    enlarge y limits  = 0.05,
    enlarge x limits  = 0.5,
    width=0.3\textwidth,
    bar width=2mm,
    symbolic y coords = {$SpaceSize_{log}$, $Shape_{log}$, $Density_{log}$, $Gini-U$, $Gini-I$, $AvgDegreee-U_{log}$, $AvgDegreee-I_{log}$, $AvgClustC-U_{log}$,$AvgClustC-I_{log}$,$Assort-U$,$Assort-I$},
    nodes near coords={
   \pgfmathprintnumber[fixed zerofill, precision=3] % <---
   {\pgfplotspointmeta}
   },
   every node near coord/.style={/pgf/number format/fixed},
   nodes near coords style = {font=\footnotesize}
  ]
  \addplot coordinates { (0.192,$SpaceSize_{log}$) (-0.231,$Shape_{log}$) (0.298,$Density_{log}$) (0.104,$Gini-U$) (0.681,$Gini-I$) (0.605,$AvgDegreee-U_{log}$) (0.374,$AvgDegreee-I_{log}$) (0.665,$AvgClustC-U_{log}$) (0.332,$AvgClustC-I_{log}$) (0.024,$Assort-U$) (-0.031,$Assort-I$)};
  \end{axis}
\end{tikzpicture}

\pgfplotsset{width=.95\textwidth, compat=newest} 

\pgfplotsset{
    discard if/.style 2 args={
        x filter/.code={
            \edef\tempa{\thisrow{#1}}
            \edef\tempb{#2}
            \ifx\tempa\tempb
                \def\pgfmathresult{inf}
            \fi
        }
    },
    discard if not/.style 2 args={
        x filter/.code={
            \edef\tempa{\thisrow{#1}}
            \edef\tempb{#2}
            \ifx\tempa\tempb
            \else
                \def\pgfmathresult{inf}
            \fi
        }
    }
}




\pgfplotstablegetrowsof{data.csv}

\edef\numberofrows{\pgfplotsretval}

\begin{tikzpicture}
\begin{axis}[
/pgf/number format/.cd,1000 sep={},
xbar,/pgf/bar shift=0pt,
y axis line style = { opacity = 0 },
axis x line       = none,
xtick=\empty,
ytick={0,...,\numberofrows}, 
y dir=reverse,
xlabel= {},
y tick label style={major tick length=0pt},
enlarge y limits  = 0.05,
enlarge x limits  = 0.5,
width=0.3\textwidth,
bar width=2mm,
yticklabels from table={data.csv}{[index]1},
nodes near coords={
   \pgfmathprintnumber[fixed zerofill, precision=3] % <---
   {\pgfplotspointmeta}
   },
   every node near coord/.style={/pgf/number format/fixed},
   nodes near coords style = {font=\footnotesize}
]
\addplot [draw,fill=blue!30] table [
    y expr=\coordindex,
    x index=0,col sep=comma
]{data.csv};

\end{axis}
\end{tikzpicture}

==> framework/main.tex <==
\begin{algorithm}[!t]
\SetAlgoLined
\textbf{Input:} Bipartite user-item graph $\mathcal{G}$, number of samples $M$.\\
\textbf{Output:} $M$ sampled graphs.\\
$m \leftarrow 1$\\
$\mathcal{M} = \{\}$\\
\While{$m \leq M$}{
    % \texttt{// get dropout rate}\\
    $\mu \leftarrow uniform([0.7, 0.9])$\\
    % \texttt{// choose graph sampling strategy}\\
    $\texttt{\textit{sampling}} \leftarrow uniform(\{\texttt{nodeDropout}, \texttt{edgeDropout}\})$\\
    % \texttt{// add sampled graph to the set}\\
    $\mathcal{M} \leftarrow \mathcal{M} \cup sample(\mathcal{G}, \mu, \texttt{\textit{sampling}})$\\
    % \texttt{// increment number of generated samples}\\
    $m \leftarrow m + 1$
}
Return $\mathcal{M}$.
\caption{Sub-dataset generation.}
\label{alg:data-generation}
\end{algorithm}

==> framework/sampling.tex <==
\begin{algorithm}[!t]
\caption{Graph sampling}
\label{alg:sampling}
\SetAlgoLined
\textbf{Input:} Bipartite user-item graph $\mathcal{G}$, dropout rate $\mu$, graph sampling strategy \texttt{\textit{sampling}}.\\
\textbf{Output:} Sampled graph $\mathcal{G}_m$.\\
\uIf{\texttt{sampling} $==$ \texttt{nodeDropout}}{
    %\texttt{// calculate nodes to sample according to} $d$\\
    $N = (U + I) * (1 - \mu)$ \\
    %\texttt{// sample $N$ nodes}\\
    $\mathcal{V}_m \leftarrow uniform_N(\mathcal{U} \cup \mathcal{I})$\\
    %\texttt{// mask $\mathbf{A}$ according to $\mathcal{V}_m$}\\
    $\mathbf{A}_m \leftarrow mask_{node}(\mathbf{A}, \mathcal{V}_m)$
}
\uElseIf{\texttt{sampling} $==$ \texttt{edgeDropout}}{
    %\texttt{// calculate edges to sample according to} $d$\\
    $N = E * (1 - \mu)$ \\
    %\texttt{// sample $N$ edges}\\
    $\mathcal{E}_m \leftarrow uniform_N(\mathcal{E}_{u \rightarrow i})$\\
    %\texttt{// mask $\mathbf{A}$ according to $\mathcal{E}_m$}\\
    $\mathbf{A}_m \leftarrow mask_{edge}(\mathbf{A}, \mathcal{E}_m)$\\
    %\texttt{// induce the set of nodes $\mathcal{V}_m$}\\
    $\mathcal{V}_m \leftarrow induce(\mathbf{A}_m)$
}
\phantom{ }\\
%\texttt{// induce $\mathcal{G}_m$ through $\mathcal{V}_m$ and $\mathbf{A}_m$}\\
$\mathcal{G}_m \leftarrow \{\mathcal{V}_m, \mathbf{A}_m\}$ \\
Return $\mathcal{G}_m$.
\end{algorithm}

==> sections/experimental_settings.tex <==
\section{Experimental settings}
EXPERIMENTAL SETTINGS

==> sections/results.tex <==
\section{Results and discussion}
RESULTS AND DISCUSSION

==> tables/add_rq1.tex <==
\begin{table}[!h]
\caption{Additional results for RQ1 on Amazon-Book. The current table is to be interpreted the same way as Table \ref{tab:rq1}.}
\label{tab:rq1_app}
% \begin{adjustbox}{width=0.6\textwidth,center}
    \centering
    \begin{tabular}{l|c|c|c|c}
    \toprule
        \multicolumn{1}{c}{\textbf{Characteristics}} & \multicolumn{1}{c}{\textbf{LightGCN}} & \multicolumn{1}{c}{\textbf{DGCF}} & \multicolumn{1}{c}{\textbf{UltraGCN}} & \multicolumn{1}{c}{\textbf{SVD-GCN}} \\ \cmidrule{1-5} 
        \rowcolor{gray} \ $R^{2}$(adj. $R^{2}$) & $0.953 (0.952)$ & $0.951 (0.950)$ & $0.800 (0.797)$& $0.964 (0.963)$
 \\ \
         $Constant$ & $0.088^{***}$&$0.079^{***}$&$0.056^{***}$&$0.112^{***}$
 \\ \
         $SpaceSize_{log}$ & $0.456^{***}$& $0.364^{***}$& $0.067^{}$& $0.433^{***}$
 \\ \
         $Shape_{log}$ &$-0.668^{***}$&$-0.598^{***}$&$-0.215^{}$&$-0.582^{***}$
 \\ \
         $Density_{log}$ & $0.546^{***}$& $0.453^{***}$& $0.141^{**}$&$0.541^{***}$
 \\ \
         $Gini\text{-}U$ &$-0.073^{}$&$-0.085^{}$&$-0.350^{**}$&$-0.042^{}$
 \\ \
         $Gini\text{-}I$ & $1.302^{***}$& $1.148^{***}$& $0.772^{***}$&$1.306^{***}$
 \\ \
         $AvgDegree\text{-}U_{log}$ &$1.336^{***}$&$1.116^{***}$&$0.316^{*}$&$1.265^{***}$
 \\ \
         $AvgDegree\text{-}I_{log}$ & $0.668^{***}$& $0.518^{***}$& $0.101^{}$& $0.683^{***}$
 \\ \
         $AvgClustC\text{-}U_{log}$ &$1.627^{***}$&$1.307^{***}$&$0.210^{}$&$1.617^{***}$
 \\ \
         $AvgClustC\text{-}I_{log}$ &$0.431^{***}$&$0.337^{***}$& $0.111^{}$& $0.354^{***}$
 \\ \
        $Assort\text{-}U$ &$0.031^{}$&$0.041^{*}$&$0.070^{***}$&$0.028^{}$
 \\ \
         $Assort\text{-}I$ &$-0.010^{}$& $-0.004^{}$& $0.025^{***}$& $-0.010^{*}$ \\ 
   \bottomrule
 \multicolumn{5}{l}{\textit{***p-value $\leq$ 0.001, **p-value $\leq$ 0.01, *p-value $\leq$ 0.05}}
    \end{tabular}
% \end{adjustbox}
\end{table}

==> tables/add_rq1_ndcg.tex <==
\begin{table}[!h]
\caption{Additional results for RQ1 on Yelp2018, Gowalla, and Amazon-Book when considering the \textit{nDCG@20} as accuracy metric. The current table is to be interpreted the same way as Table \ref{tab:rq1}, but \textit{nDCG@20} is the recommendation metric this time.}
\label{tab:rq1_ndcg}
    \centering
    % \begin{adjustbox}{width=\textwidth,center}
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
    \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Characteristics}}} & \multicolumn{3}{c}{\textbf{LightGCN}} & \multicolumn{3}{c}{\textbf{DGCF}} & \multicolumn{3}{c}{\textbf{UltraGCN}} & \multicolumn{3}{c}{\textbf{SVD-GCN}} \\ \cmidrule{2-13}
        \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Yelp2018}} & \textbf{Amazon-Book} & \multicolumn{1}{c}{\textbf{Gowalla}} & \textbf{Yelp2018} & \textbf{Amazon-Book} & \multicolumn{1}{c}{\textbf{Gowalla}} & \textbf{Yelp2018} & \textbf{Amazon-Book} & \multicolumn{1}{c}{\textbf{Gowalla}} & \textbf{Yelp2018} & \textbf{Amazon-Book} & \textbf{Gowalla} \\ \cmidrule{1-13}
        \rowcolor{gray} $R^{2}$(adj. $R^{2}$) & $0.971 (0.970)$& $0.947 (0.946)$& $0.978 (0.977)$& $0.972 (0.971)$& $0.945 (0.944)$& $0.980 (0.979)$& $0.966 (0.966)$& $0.748 (0.743)$& $0.865 (0.863)$& $0.982 (0.982)$& $0.958 (0.957)$& $0.980 (0.980)$ \\ \
         $Constant$ & $0.048^{***}$&$0.043^{***}$&$0.068^{***}$&$0.043^{***}$&$0.039^{***}$&$0.061^{***}$&$0.028^{***}$&$0.025^{***}$&$0.034^{***}$&$0.056^{***}$&$0.054^{***}$&$0.076^{***}$ \\ \
         $SpaceSize_{log}$ & $0.054^{***}$& $0.286^{***}$& $0.142^{***}$& $0.086^{***}$& $0.229^{***}$& $0.170^{***}$& $-0.017^{**}$& $0.054^{}$& $0.216^{***}$& $0.062^{***}$& $0.290^{***}$& $0.107^{***}$ \\ \
         $Shape_{log}$ & $-0.191^{***}$&$-0.447^{***}$&$-0.168^{*}$&$-0.185^{***}$&$-0.389^{***}$&$-0.134^{}$&$0.062^{}$&$-0.154^{}$&$-0.019^{}$&$-0.159^{**}$&$-0.417^{***}$&$-0.193^{*}$ \\ \
         $Density_{log}$ &  $0.115^{***}$& $0.332^{***}$& $0.199^{***}$& $0.140^{***}$& $0.274^{***}$& $0.218^{***}$& $0.024^{***}$& $0.090^{**}$& $0.213^{***}$& $0.131^{***}$& $0.345^{***}$& $0.172^{***}$
 \\ \
         $Gini\text{-}U$ & $0.140^{**}$&$-0.106^{}$&$-0.034^{}$&$0.046^{}$&$-0.105^{}$&$-0.085^{}$&$0.060^{}$&$-0.194^{**}$&$-0.547^{***}$&$0.050^{}$&$-0.140^{*}$&$0.012^{}$
 \\ \
         $Gini\text{-}I$ & $0.678^{***}$& $0.720^{***}$& $0.438^{***}$& $0.588^{***}$& $0.624^{***}$& $0.368^{***}$& $0.264^{***}$& $0.393^{***}$& $-0.145^{}$& $0.561^{***}$& $0.722^{***}$& $0.482^{***}$
 \\ 
         $AvgDegree\text{-}U_{log}$ & $0.264^{***}$&$0.841^{***}$&$0.425^{***}$&$0.319^{***}$&$0.698^{***}$&$0.455^{***}$&$-0.024^{}$&$0.221^{*}$&$0.439^{***}$&$0.273^{***}$&$0.843^{***}$&$0.375^{***}$
 \\ \
         $AvgDegree\text{-}I_{log}$ & $0.073^{*}$& $0.394^{***}$& $0.257^{***}$& $0.134^{***}$& $0.309^{***}$& $0.322^{***}$& $0.038^{}$& $0.068^{}$& $0.420^{***}$& $0.113^{***}$& $0.426^{***}$& $0.182^{***}$
 \\ \
         $AvgClustC\text{-}U_{log}$ & $0.405^{***}$&$1.050^{***}$&$0.514^{***}$&$0.466^{***}$&$0.843^{***}$&$0.551^{***}$&$-0.006^{}$&$0.167^{}$&$0.461^{***}$&$0.441^{***}$&$1.094^{***}$&$0.443^{***}$
 \\ \
         $AvgClustC\text{-}I_{log}$ & $0.024^{}$& $0.205^{***}$& $0.193^{}$& $0.070^{}$& $0.163^{**}$& $0.258^{**}$& $0.038^{}$& $0.062^{}$& $0.461^{***}$& $0.016^{}$& $0.174^{**}$& $0.146^{}$
 \\ \
          $Assort\text{-}U$ & $0.058^{***}$&$0.018^{}$&$0.020^{**}$&$0.055^{***}$&$0.022^{*}$&$0.014^{*}$&$0.093^{***}$&$0.045^{***}$&$0.005^{}$&$0.048^{***}$&$0.016^{}$&$0.008^{}$
 \\ \
         $Assort\text{-}I$ & $-0.029^{*}$& $-0.005^{}$& $-0.034^{}$& $-0.029^{*}$& $-0.002^{}$& $-0.046^{}$& $0.005^{}$& $0.016^{***}$& $-0.113^{***}$& $-0.028^{*}$& $-0.006^{*}$& $-0.074^{**}$
 \\ 
   \bottomrule
 \multicolumn{13}{l}{\textit{***p-value $\leq$ 0.001, **p-value $\leq$ 0.01, *p-value $\leq$ 0.05}}
    \end{tabular}
    % \end{adjustbox}
\end{table}

==> tables/add_rq2.tex <==
\begin{table}[!h]
\caption{Additional results for RQ2 on DGCF and UltraGCN. The current table is to be interpreted the same way as Table \ref{tab:rq2}.}
\label{tab:rq2_app}
% \begin{adjustbox}{width=\textwidth,center}
    \centering
    \begin{tabular}{l|cc|cc|cc|cc}
    \toprule
         \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Node drop} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=black]{2.5pt} \quad
         \textbf{Edge drop} \tikzcircle[fill=white]{2.5pt} \tikzcircle[fill=white]{2.5pt} \tikzcircle[fill=white]{2.5pt}} & \multicolumn{2}{c}{\textbf{Node drop} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=white]{2.5pt} \quad
         \textbf{Edge drop} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=white]{2.5pt} \tikzcircle[fill=white]{2.5pt}} & \multicolumn{2}{c}{\textbf{Node drop} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=white]{2.5pt} \tikzcircle[fill=white]{2.5pt} \quad
         \textbf{Edge drop} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=white]{2.5pt}} & \multicolumn{2}{c}{\textbf{Node drop} \tikzcircle[fill=white]{2.5pt} \tikzcircle[fill=white]{2.5pt} \tikzcircle[fill=white]{2.5pt} \quad
         \textbf{Edge drop} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=black]{2.5pt} \tikzcircle[fill=black]{2.5pt}} \\ \cmidrule{2-9}
         \multicolumn{1}{c}{} & \multicolumn{2}{c}{\makecell[c]{\textit{\ul{Average Sampling Statistics}}\\\textbf{Users:} 5,828 \quad \textbf{Items:} 7,887 \\ \textbf{Interactions:} 45,620}} & \multicolumn{2}{c}{\makecell[c]{\textit{\ul{Average Sampling Statistics}}\\\textbf{Users:} 12,744 \quad \textbf{Items:} 17,229 \\ \textbf{Interactions:} 97,785}} & \multicolumn{2}{c}{\makecell[c]{\textit{\ul{Average Sampling Statistics}}\\\textbf{Users:} 21,730 \quad \textbf{Items:} 29,316 \\ \textbf{Interactions:} 160,919\\}} & \multicolumn{2}{c}{\makecell[c]{\textit{\ul{Average Sampling Statistics}}\\\textbf{Users:} 28,526 \quad \textbf{Items:} 38,467 \\ \textbf{Interactions:} 209,659}} \\ \cmidrule{2-9} 
         \multicolumn{1}{c}{\textbf{Characteristics}} & \multicolumn{1}{c}{\textbf{DGCF}} & \multicolumn{1}{c}{\textbf{UltraGCN}} & \multicolumn{1}{c}{\textbf{DGCF}} & \multicolumn{1}{c}{\textbf{UltraGCN}} & \multicolumn{1}{c}{\textbf{DGCF}} & \multicolumn{1}{c}{\textbf{DGCF}} & \multicolumn{1}{c}{\textbf{UltraGCN}} \\ 
         \cmidrule{1-9} 
         \rowcolor{gray} $R^{2}$(adj. $R^{2}$) &$0.888 (0.884)$&$0.597 (0.583)$ &$0.973 (0.972)$&$0.833 (0.827)$&$0.988 (0.988)$&$0.883 (0.879)$&$0.994 (0.994)$&$0.599 (0.584)$ \\
        $Constant$ &$0.162^{***}$&$0.091^{***}$&$0.131^{***}$&$0.074^{***}$&$0.085^{***}$&$0.051^{***}$&$0.051^{***}$&$0.034^{***}$ \\
        $SpaceSize_{log}$ &$0.130^{**}$&$0.175^{*}$&$0.192^{***}$&$0.358^{***}$&$0.264^{***}$&$0.337^{***}$&$-0.188^{***}$&$1.644^{***}$ \\
        $Shape_{log}$ &$-0.109^{}$&$-0.096^{}$&$-0.232^{*}$&$-0.022^{}$&$-0.136^{}$&$-0.029^{}$&$-0.011^{}$&$1.055^{**}$ \\
        $Density_{log}$ &$-0.005^{}$&$0.394^{***}$&$0.294^{***}$&$0.355^{***}$&$0.351^{***}$&$0.340^{***}$&$0.168^{***}$&$0.185^{}$ \\
        $Gini\text{-}U$ &$-0.136^{}$&$-0.824^{***}$&$0.083^{}$&$-0.880^{***}$&$0.130^{}$&$-0.775^{**}$&$0.200^{*}$&$-0.961^{}$ \\
        $Gini\text{-}I$ &$0.756^{***}$&$-0.152^{}$&$0.717^{***}$&$-0.248^{}$&$0.668^{***}$&$-0.333^{}$&$0.264^{**}$&$-0.732^{}$ \\
        $AvgDegree\text{-}U_{log}$ &$0.179^{**}$&$0.617^{***}$&$0.601^{***}$&$0.723^{***}$&$0.684^{***}$&$0.692^{***}$&$-0.014^{}$&$1.302^{***}$\\
        $AvgDegree\text{-}I_{log}$ &$0.070^{}$&$0.521^{**}$&$0.369^{***}$&$0.702^{***}$&$0.547^{***}$&$0.663^{***}$&$-0.025^{}$&$2.356^{***}$ \\
        $AvgClustC\text{-}U_{log}$ &$0.362^{***}$&$0.619^{**}$&$0.715^{***}$&$0.641^{**}$&$0.706^{***}$&$0.481^{}$&$0.001^{}$&$1.099^{**}$\\
        $AvgClustC\text{-}I_{log}$ &$-0.080^{}$&$0.412^{}$&$0.252^{}$&$0.903^{**}$&$0.571^{**}$&$0.962^{**}$&$-0.083^{}$&$2.415^{***}$ \\
        $Assort\text{-}U$ &$-0.001^{}$&$0.001^{}$&$0.011^{}$&$0.000^{}$&$0.001^{}$&$0.012^{}$&$0.008^{}$&$0.064^{}$ \\
        $Assort\text{-}I$ &$-0.050^{}$&$-0.111^{**}$&$0.002^{}$&$-0.151^{**}$&$0.002^{}$&$-0.086^{}$&$-0.032^{}$&$-0.141^{}$
         \\
    \bottomrule
    \multicolumn{9}{l}{\textit{***p-value $\leq$ 0.001, **p-value $\leq$ 0.01, *p-value $\leq$ 0.05}}
    \end{tabular}
    % \end{adjustbox}
\end{table}

==> tables/chars_legend.tex <==
\begin{table}[!b]
\caption{Selected \textit{classical} and \textit{topological} characteristics. We report the full name, the symbol, whether it is rescaled via log10, and the shorthand adopted.}
\label{tab:shorthand}
% \begin{adjustbox}{width=0.8\textwidth,center}
\begin{tabular}{l|l|c|c|l}
\toprule
\multicolumn{1}{l}{\textbf{Type}} & \multicolumn{1}{l}{\textbf{Characteristics}} & \multicolumn{1}{l}{\textbf{Symbol}} & \multicolumn{1}{l}{\textbf{Log10}} & \multicolumn{1}{l}{\textbf{Shorthand}} \\
 \cmidrule{1-5}
\multirow{5}{*}{\textit{Classical}} & {Space size} & {$\zeta$} & {\checkmark} & {$SpaceSize_{log}$} \\
 & Shape & $\pi$ & \checkmark & $Shape_{log}$ \\
 & {Density} & {$\delta$} & {\checkmark} & {$Density_{log}$} \\
 & Gini user & $\kappa_{\mathcal{U}}$ &  & $Gini\text{-}U$ \\
 & {Gini item} & {$\kappa_{\mathcal{I}}$} & {} & {$Gini\text{-}I$} \\
 \hline
\multirow{6}{*}{\textit{Topological}} & {Average degree user} & {$\sigma_{\mathcal{U}}$} & {\checkmark} & {$AvgDegree\text{-}U_{log}$} \\
 & Average degree item & $\sigma_{\mathcal{I}}$ & \checkmark & $AvgDegree\text{-}I_{log}$ \\
 & {Average clustering coefficient user} & {$\gamma_{\mathcal{U}}$} & {\checkmark} & {$AvgClustC\text{-}U_{log}$} \\
 & Average clustering coefficient item & $\gamma_{\mathcal{I}}$ & \checkmark & $AvgClustC\text{-}I_{log}$ \\
 & {Degree assortativity user} & {$\rho_{\mathcal{U}}$} & {} & {$Assort\text{-}U$} \\
 & Degree assortativity item & $\rho_{\mathcal{I}}$ &  & $Assort\text{-}I$\\
\bottomrule
\end{tabular}
% \end{adjustbox}
\end{table}

==> tables/chars_values.tex <==
\begin{table}[!b]
\caption{Dataset overall statistics and characteristic aggregated statistics (minimum and maximum values, mean, and standard deviation) on the sampled sub-datasets.}
\label{tab:dataset-chars}
% \begin{adjustbox}{width=1\textwidth,center}
    \begin{tabular}{l|cccc|cccc|cccc}
    \toprule
        \multicolumn{1}{c}{} & \multicolumn{4}{c}{\textbf{Yelp2018}} & \multicolumn{4}{c}{\textbf{Amazon-Book}} & \multicolumn{4}{c}{\textbf{Gowalla}} \\ \cmidrule{2-13}
        \multicolumn{1}{c}{} & \multicolumn{4}{c}{\makecell[c]{\textit{\ul{Overall Statistics}}\\\textbf{Users:} 25,677 \quad \textbf{Items:} 25,815\\\textbf{Interactions:} 696,865}} & \multicolumn{4}{c}{\makecell[c]{\textit{\ul{Overall Statistics}}\\\textbf{Users:} 70,679 \quad \textbf{Items:} 24,915\\\textbf{Interactions:} 846,434}} & \multicolumn{4}{c}{\makecell[c]{\textit{\ul{Overall Statistics}}\\\textbf{Users:} 29,858 \quad \textbf{Items:} 40,981\\\textbf{Interactions:} 1,027,370}} \\ \cmidrule{2-13}
        \multicolumn{1}{c}{\textbf{Characteristics}} & \textbf{Min} & \textbf{Max} & \textbf{Mean} & \multicolumn{1}{c}{\textbf{Std}} & \textbf{Min} & \multicolumn{1}{c}{\textbf{Max}} & \textbf{Mean} & \multicolumn{1}{c}{\textbf{Std}} & \textbf{Min} & \multicolumn{1}{c}{\textbf{Max}} & \textbf{Mean} & \textbf{Std} \\
        \cmidrule{1-13}  
        $SpaceSize_{log}$ & 0.256 & 1.393 & 1.000 & 0.379 & 0.405 & 1.593 & 1.176 & 0.384 & 0.430 & 1.541 & 1.161 & 0.375 \\
        $Shape_{log}$ & 0.019 & 0.105 & 0.045 & 0.014 & 0.325 & 0.443 & 0.407 & 0.021 & -0.149 & -0.097 & -0.129 & 0.008 \\ 
        $Density_{log}$ & -3.699 & -2.693 & -3.219 & 0.358 & -3.902 & -2.896 & -3.497 & 0.365 & -3.889 & -2.876 & -3.380 & 0.363 \\ 
        $Gini\text{-}U$ & 0.443 & 0.508 & 0.486 & 0.008 & 0.384 & 0.499 & 0.459 & 0.023 & 0.462 & 0.512 & 0.491 & 0.007 \\ 
        $Gini\text{-}I$ & 0.500 & 0.609 & 0.575 & 0.019 & 0.518 & 0.618 & 0.586 & 0.018 & 0.437 & 0.502 & 0.478 & 0.008 \\ 
        $AvgDegree\text{-}U_{log}$ & 0.523 & 0.926 & 0.758 & 0.110 & 0.318 & 0.609 & 0.476 & 0.077 & 0.603 & 1.017 & 0.846 & 0.115 \\ 
        $AvgDegree\text{-}I_{log}$ & 0.565 & 0.955 & 0.804 & 0.098 & 0.682 & 1.043 & 0.883 & 0.096 & 0.487 & 0.888 & 0.717 & 0.109 \\ 
        $AvgClustC\text{-}U_{log}$ & -1.144 & -0.662 & -0.947 & 0.126 & -0.757 & -0.407 & -0.602 & 0.095 & -1.211 & -0.741 & -1.013 & 0.122 \\ 
        $AvgClustC\text{-}I_{log}$ & -1.092 & -0.652 & -0.922 & 0.105 & -1.124 & -0.751 & -0.967 & 0.099 & -1.080 & -0.614 & -0.881 & 0.124 \\ 
        $Assort\text{-}U$ & -0.051 & 0.235 & 0.021 & 0.035 & -0.041 & 0.533 & 0.052 & 0.074 & 0.042 & 0.544 & 0.188 & 0.071 \\ 
        $Assort\text{-}I$ & -0.002 & 0.237 & 0.067 & 0.037 & 0.000 & 0.842 & 0.443 & 0.264 & -0.037 & 0.161 & 0.021 & 0.028 \\ \bottomrule
    \end{tabular}
    % \end{adjustbox}
\end{table}

==> tables/models.tex <==
\begin{table}[!t]
\caption{Selected models for our study. For each of them, we report year, works using them as baselines, and strategy.}
%\rowcolors{1}{}{gray!15}
%\begin{adjustbox}{width=1\columnwidth,center}
% \begin{adjustbox}{width=1\textwidth,center}
\begin{tabular}{l|c|c|l}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Year}} & \multicolumn{1}{c}{\begin{tabular}{c}\textbf{Baseline in}\\\textbf{(2021-)}\end{tabular}} & \multicolumn{1}{c}{\textbf{Strategy}}
\\\cmidrule{1-4}
LightGCN~\cite{DBLP:conf/sigir/0001DWLZ020} & 2020 & e.g.,~\cite{DBLP:conf/sigir/WuWF0CLX21, DBLP:conf/www/LiuCZGN21, DBLP:conf/sigir/YuY00CN22, DBLP:conf/sigir/XiaHXZYH22, DBLP:conf/kdd/RaoCLSYH22} & \begin{tabular}{l} 
$\bullet$ Removes feature transformation \\
$\bullet$ Removes non-linearities
\end{tabular} \\ \hline 
DGCF~\cite{DBLP:conf/sigir/WangJZ0XC20} & 2020 & e.g.,~\cite{ DBLP:conf/sigir/ZhangL0WSLSZDZ22, DBLP:conf/sigir/FanL0ZT022, 9736612, DBLP:conf/wsdm/WangZS22, DBLP:conf/www/LinTHZ22} & \begin{tabular}{l}
\makecell[l]{$\bullet$ Disentangles users' and items' into intents and weights their importance} \\ 
\makecell[l]{$\bullet$ Updates graph structure according to those learned intents}
\end{tabular} \\ \hline 
UltraGCN~\cite{DBLP:conf/cikm/MaoZXLWH21} & 2021 & e.g.,~\cite{DBLP:conf/mm/DuWF0022, DBLP:conf/cikm/GongSWLL22, DBLP:conf/sigir/ZhuDSMLCXZ22,DBLP:conf/sigir/0001OM22, 10.1145/3570501} & \begin{tabular}{l}
\makecell[l]{$\bullet$ Approximates infinite propagation layers through a constraint loss and negative sampling} \\
$\bullet$ Explores item-item connections
\end{tabular}\\ \hline 
SVD-GCN~\cite{DBLP:conf/cikm/PengSM22} & 2022 & e.g.,~\cite{DBLP:journals/corr/abs-2306-02259, DBLP:journals/corr/abs-2306-04370} & \begin{tabular}{l}
\makecell[l]{$\bullet$ Approximates GCN propagation layers through truncated SVD}\\
$\bullet$ Explores user-user connections\\
$\bullet$ Explores item-item connections
\end{tabular}\\
 \bottomrule
 \end{tabular}
\label{tab:models}
% \end{adjustbox}
\end{table}

==> tables/models_degree.tex <==
\begin{table*}[!t]
\centering
\caption{Selected models for our study. For each of them, we report year, works using them as baselines, and which \textit{topological} characteristics are integrated in the models' formulations.}
\footnotesize
\setlength{\tabcolsep}{10pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5} % Default value: 1
\begin{tabular}{lccl}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Year}} & \multicolumn{1}{c}{\textbf{Baseline in (2021-)}} & \multicolumn{1}{c}{\textbf{Topological characteristics}} \\ \hline
LightGCN~\cite{DBLP:conf/sigir/0001DWLZ020} & 2020 & e.g.,~\cite{DBLP:conf/sigir/WuWF0CLX21, DBLP:conf/www/LiuCZGN21, DBLP:conf/sigir/YuY00CN22, DBLP:conf/sigir/XiaHXZYH22, DBLP:conf/kdd/RaoCLSYH22} & 
\parbox[t]{5cm}{\textbf{Node degree} used to normalize the adjacency matrix in the message passing.} \\ \hline
DGCF~\cite{DBLP:conf/sigir/WangJZ0XC20} & 2020 & e.g.,~\cite{ DBLP:conf/sigir/ZhangL0WSLSZDZ22, DBLP:conf/sigir/FanL0ZT022, 9736612, DBLP:conf/wsdm/WangZS22, DBLP:conf/www/LinTHZ22} & \parbox[t]{5cm}{\textbf{Node degree} used to normalize the adjacency matrix in the message passing.} \\ \hline
UltraGCN~\cite{DBLP:conf/cikm/MaoZXLWH21} & 2021 & e.g.,~\cite{DBLP:conf/mm/DuWF0022, DBLP:conf/cikm/GongSWLL22, DBLP:conf/sigir/ZhuDSMLCXZ22,DBLP:conf/sigir/0001OM22, 10.1145/3570501} & \parbox[t]{5cm}{\textbf{Node degree} used for normalization in the infinite layer message passing. The model also learns from the \textbf{\textit{item}-projected graph}.} \\ \hline
SVD-GCN~\cite{DBLP:conf/cikm/PengSM22} & 2022 & e.g.,~\cite{DBLP:journals/corr/abs-2306-02259, DBLP:journals/corr/abs-2306-04370} & \parbox[t]{5cm}{The formulation for the node embeddings involves the largest singular values of the normalized user-item interaction matrix, whose maximum value is related to the maximum \textbf{node degree} of the user-item graph. The model also learns from the \textbf{\textit{user}-} and \textbf{\textit{item}-projected graphs}.} \\
 \bottomrule
 \end{tabular}
\label{tab:models}
\end{table*}

==> tables/results.tex <==
\begin{table*}[!t]
\caption{Results of the explanatory model with the \textit{Recall@20} as recommendation metric. Besides the row in light gray standing for the $R^2$, the other rows refer to the learned characteristics' coefficients (with the statistical significance). $Constant$ (i.e., $\theta_0$) is the expected value of \textit{Recall@20}.}
\label{tab:rq1}
% % \begin{adjustbox}{width=\textwidth,center
    \centering
    \begin{tabular}{l|cc|cc|cc|cc}
    \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Characteristics}}} & \multicolumn{2}{c}{\textbf{LightGCN}} & \multicolumn{2}{c}{\textbf{DGCF}} & \multicolumn{2}{c}{\textbf{UltraGCN}} & \multicolumn{2}{c}{\textbf{SVD-GCN}} \\ \cmidrule{2-9} \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Yelp2018}} & \multicolumn{1}{c}{\textbf{Gowalla}} & \textbf{Yelp2018} & \multicolumn{1}{c}{\textbf{Gowalla}} & \textbf{Yelp2018} & \multicolumn{1}{c}{\textbf{Gowalla}} & \textbf{Yelp2018} & \textbf{Gowalla} \\ \cmidrule{1-9}
        \rowcolor{gray} \ $R^{2}$(adj. $R^{2}$) & $0.971 (0.971)$& $0.979 (0.978)$& $0.973 (0.973)$& $0.982 (0.981)$& $0.965 (0.964)$& $0.860 (0.858)$& $0.982 (0.981)$& $0.981 (0.981)$
 \\ \
         $Constant$ & $0.100^{***}$&$0.121^{***}$&$0.089^{***}$&$0.107^{***}$&$0.061^{***}$&$0.062^{***}$&$0.116^{***}$&$0.135^{***}$
 \\ \
         $SpaceSize_{log}$ & $0.070^{***}$& $0.192^{***}$& $0.133^{***}$& $0.237^{***}$& $-0.059^{***}$& $0.318^{***}$& $0.064^{***}$& $0.114^{***}$
 \\ \
         $Shape_{log}$ & $-0.253^{*}$&$-0.231^{}$&$-0.282^{**}$&$-0.220^{*}$&$0.135^{}$&$-0.003^{}$&$-0.193^{}$&$-0.232^{*}$
 \\ \
         $Density_{log}$ & $0.194^{***}$&$0.298^{***}$& $0.243^{***}$& $0.327^{***}$& $0.026^{*}$& $0.321^{***}$& $0.203^{***}$& $0.234^{***}$
 \\ \
         $Gini\text{-}U$ & $0.296^{**}$&$0.104^{}$&$0.074^{}$&$-0.071^{}$&$-0.043^{}$&$-0.931^{***}$&$0.136^{}$&$0.143^{}$
 \\ \
         $Gini\text{-}I$ & $1.362^{***}$& $0.681^{***}$& $1.108^{***}$& $0.560^{***}$& $0.605^{***}$& $-0.144^{}$& $1.138^{***}$& $0.748^{***}$
 \\ \
         $AvgDegree\text{-}U_{log}$ & $0.390^{***}$&$0.605^{***}$&$0.518^{***}$&$0.673^{***}$&$-0.100^{*}$&$0.640^{***}$&$0.364^{***}$&$0.464^{***}$
 \\ \
         $AvgDegree\text{-}I_{log}$ & $0.137^{*}$& $0.374^{***}$& $0.235^{***}$& $0.453^{***}$& $0.034^{}$& $0.637^{***}$& $0.171^{**}$& $0.231^{**}$
 \\ \
         $AvgClustC\text{-}U_{log}$ & $0.613^{***}$&$0.665^{***}$&$0.726^{***}$&$0.783^{***}$&$-0.077^{}$&$0.706^{***}$&$0.613^{***}$&$0.496^{***}$
 \\ \
         $AvgClustC\text{-}I_{log}$ & $0.087^{}$& $0.332^{*}$& $0.168^{}$& $0.373^{**}$& $0.062^{}$& $0.671^{**}$& $0.057^{}$& $0.215^{}$
 \\ \
        $Assort\text{-}U$ & $0.094^{***}$&$0.024^{*}$&$0.093^{***}$&$0.013^{}$&$0.123^{***}$&$-0.019^{}$&$0.080^{***}$&$0.010^{}$
 \\ \
         $Assort\text{-}I$ & $-0.051^{}$& $-0.031^{}$& $-0.056^{*}$& $-0.055^{}$& $0.001^{}$& $-0.174^{***}$& $-0.048^{*}$& $-0.088^{*}$ \\ 
   \bottomrule
 \multicolumn{9}{l}{\textit{***p-value $\leq$ 0.001, **p-value $\leq$ 0.01, *p-value $\leq$ 0.05}}
    \end{tabular}
    % \end{adjustbox}
\end{table*}
